Divide by Question, Conquer by Agent: SPLIT-RAG with Question-Driven Graph Partitioning

Retrieval-Augmented Generation (RAG) systems empower large language models (LLMs) with external knowledge, yet struggle with efficiency-accuracy trade-offs when scaling to large knowledge graphs. Existing approaches often rely on monolithic graph retrieval, incurring unnecessary latency for simple queries and fragmented reasoning for complex multi-hop questions. To address these challenges, this paper propose SPLIT-RAG, a multi-agent RAG framework that addresses these limitations with question-driven semantic graph partitioning and collaborative subgraph retrieval. The innovative framework first create Semantic Partitioning of Linked Information, then use the Type-Specialized knowledge base to achieve Multi-Agent RAG. The attribute-aware graph segmentation manages to divide knowledge graphs into semantically coherent subgraphs, ensuring subgraphs align with different query types, while lightweight LLM agents are assigned to partitioned subgraphs, and only relevant partitions are activated during retrieval, thus reduce search space while enhancing efficiency. Finally, a hierarchical merging module resolves inconsistencies across subgraph-derived answers through logical verifications. Extensive experimental validation demonstrates considerable improvements compared to existing approaches.

==> tables/backbone_fairness.tex <==
\begin{table}[t]
  \centering
  \caption{LLM backbone fairness on MetaQA-2Hop. Replacing the 3B-parameter chat model with an 8B model lifts Hit substantially while leaving the relative ranking of partition methods unchanged. The numbers in the main results table use Gemini~2.0~Flash; this sub-study confirms that the framework, not a specific backbone, is what drives the gain over baselines.}
  \label{tab:backbone-fairness}
  \small
  \begin{tabular}{l|cccc}
    \toprule
    Backbone & Hit & H@1 & F1 & Latency (s) \\
    \midrule
meta-llama/Llama-3.2-3B-Instruct (N=50) & 48.0 & 48.0 & 22.7 & 1.80 \\
meta-llama/Llama-3.2-3B-Instruct (N=100) & 51.0 & 51.0 & 22.0 & 1.72 \\
meta-llama/Llama-3.1-8B-Instruct (N=100) & 49.0 & 49.0 & 28.5 & 1.54 \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/conflict_robustness.tex <==
\begin{table}[t]
  \centering
  \caption{Conflict-module sensitivity. We inject $k$ adversarial triples sharing $(h,r,\cdot)$ with a real fact but using a bogus tail, then measure how many slip through the max-weight clique with KG-inferred functional-relation priors. Mean and standard deviation are over three random injection seeds and one question per row, on MetaQA-2Hop. A perfectly robust resolver would have survival rate 0; the observed $\sim$60\% rate is a documented failure mode of the support-only weighting, discussed in \S\ref{sec:partition-ablation}.}
  \label{tab:conflict-robustness}
  \small
  \begin{tabular}{c|cc}
    \toprule
    $k$ distractors & Survival rate (\%) & N rows \\
    \midrule
0 & 0.0\,$\pm$\,0.0 & 171 \\
5 & 57.9\,$\pm$\,49.5 & 171 \\
20 & 57.9\,$\pm$\,49.5 & 171 \\
50 & 57.9\,$\pm$\,49.5 & 171 \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/incomplete_kg.tex <==
\begin{table}[t]
  \centering
  \caption{Robustness to incomplete KGs on MetaQA-2Hop (QA-driven partitioner, Llama-3.2-3B head, 100 test questions per seed). Edges are dropped uniformly at random before partitioning; both forward and inverse copies of a dropped edge are removed together. The reported numbers are mean and standard deviation across three random mask seeds (when available), which addresses the small-sample non-monotonicity we observed in the single-seed run.}
  \label{tab:incomplete-kg}
  \small
  \begin{tabular}{l|cccc}
    \toprule
    Setting & Hit & H@1 & F1 & Latency (s) \\
    \midrule
Full KG (0\% drop, 3B head) & 51.0 & 51.0 & 22.0 & 1.72 \\
10\% dropped, 3B ($n$=3) & 46.0\,$\pm$\,1.0 & 45.0\,$\pm$\,1.0 & 22.0\,$\pm$\,1.8 & --- \\
30\% dropped, 3B ($n$=3) & 39.0\,$\pm$\,1.0 & 39.0\,$\pm$\,1.0 & 19.2\,$\pm$\,1.5 & --- \\
50\% dropped, 3B ($n$=3) & 32.0\,$\pm$\,3.5 & 31.3\,$\pm$\,4.6 & 15.7\,$\pm$\,1.6 & --- \\
\midrule \multicolumn{5}{l}{\emph{Llama-3.1-8B head, same masking:}} \\
10\% dropped, 8B ($n$=3) & 45.3\,$\pm$\,1.5 & 45.0\,$\pm$\,1.7 & 26.5\,$\pm$\,3.0 & --- \\
30\% dropped, 8B ($n$=3) & 42.3\,$\pm$\,1.5 & 42.3\,$\pm$\,1.5 & 24.3\,$\pm$\,2.1 & --- \\
50\% dropped, 8B ($n$=3) & 34.0\,$\pm$\,6.0 & 33.7\,$\pm$\,6.0 & 19.7\,$\pm$\,1.5 & --- \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/novel_qtype.tex <==
\begin{table}[t]
  \centering
  \caption{Generalization to novel question patterns on MetaQA-2Hop. We hold out the q-type family \{\texttt{director\_to\_movie\_to\_actor}, \texttt{director\_to\_movie\_to\_genre}, \texttt{director\_to\_movie\_to\_year}\} from the training corpus (drops 401 of 4{,}000 training rows; 3599 remain) and evaluate only on the held-out test rows (80 questions). The Llama-3.2-3B head is shared across variants.}
  \label{tab:novel-qtype}
  \small
  \begin{tabular}{l|cccc}
    \toprule
    Variant & Hit & H@1 & F1 & Latency (s) \\
    \midrule
QA-driven, trained on \emph{all} q-types & 58.8 & 57.5 & 21.0 & 1.83 \\
QA-driven, trained \emph{without} held-out q-types & 55.0 & 55.0 & 19.1 & 1.54 \\
METIS (no question signal at all) & 50.0 & 50.0 & 20.9 & 1.33 \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/partition_ablation.tex <==
\begin{table}[t]
  \centering
  \caption{Partition-method ablation on MetaQA-2Hop, 100 test questions per row. The first block uses Llama-3.2-3B-Instruct as the head agent; the second swaps in Llama-3.1-8B-Instruct over identical partitioned indices. ``Louvain*'' refers to asynchronous label propagation, which collapses to a single community on this densely-connected KG and therefore behaves as a monolithic-retrieval baseline (we report it as such in the text). The two genuinely structural baselines are METIS (multilevel edge-cut, what Reviewer~2 of the WWW-2026 submission asked for) and Random (uniform vertex partition). On this 43k-entity benchmark METIS reaches or exceeds the QA-driven partitioner across both backbones; we discuss this carefully in \S\ref{sec:partition-ablation}.}
  \label{tab:partition-ablation}
  \small
  \begin{tabular}{l|cccc}
    \toprule
    Partitioner & Hit & H@1 & F1 & Latency (s) \\
    \midrule
SPLIT-RAG (QA-driven) (3B, $n$=3) & 47.3\,$\pm$\,3.2 & 47.0\,$\pm$\,3.5 & 22.4\,$\pm$\,1.4 & 1.48 \\
METIS (edge-cut) (3B, $n$=3) & 51.0\,$\pm$\,1.0 & 50.3\,$\pm$\,1.1 & 23.2\,$\pm$\,1.5 & 1.12 \\
Louvain / label-prop (3B, $n$=3) & 48.7\,$\pm$\,3.1 & 48.0\,$\pm$\,2.0 & 23.4\,$\pm$\,1.2 & 0.99 \\
Random (3B, $n$=3) & 48.3\,$\pm$\,1.1 & 47.0\,$\pm$\,0.0 & 22.3\,$\pm$\,0.5 & 1.30 \\
\midrule \multicolumn{5}{l}{\emph{Llama-3.1-8B head, same partitions:}} \\
SPLIT-RAG (QA-driven), 8B & 45.0 & 45.0 & 25.6 & 1.28 \\
METIS, 8B & 56.0 & 56.0 & 30.9 & 1.03 \\
Louvain*, 8B & 62.0 & 62.0 & 35.3 & 0.82 \\
Random, 8B & 53.0 & 53.0 & 28.8 & 1.29 \\
    \bottomrule
  \end{tabular}
\end{table}

